To Drop or Not to Drop: Robustness, Consistency and Differential Privacy Properties of Dropout

Training deep belief networks (DBNs) requires optimizing a non-convex function with an extremely large number of parameters. Naturally, existing gradient descent (GD) based methods are prone to arbitrarily poor local minima. In this paper, we rigorously show that such local minima can be avoided (upto an approximation error) by using the dropout technique, a widely used heuristic in this domain. In particular, we show that by randomly dropping a few nodes of a one-hidden layer neural network, the training objective function, up to a certain approximation error, decreases by a multiplicative factor. On the flip side, we show that for training convex empirical risk minimizers (ERM), dropout in fact acts as a "stabilizer" or regularizer. That is, a simple dropout based GD method for convex ERMs is stable in the face of arbitrary changes to any one of the training points. Using the above assertion, we show that dropout provides fast rates for generalization error in learning (convex) generalized linear models (GLM). Moreover, using the above mentioned stability properties of dropout, we design dropout based differentially private algorithms for solving ERMs. The learned GLM thus, preserves privacy of each of the individual training points while providing accurate predictions for new test points. Finally, we empirically validate our stability assertions for dropout in the context of convex ERMs and show that surprisingly, dropout significantly outperforms (in terms of prediction accuracy) the L2 regularization based methods for several benchmark datasets.

==> tex/appBackground.tex <==
\subsection{Gaussian mechanism for differential privacy}
\label{app:background}

\mypar{Gaussian mechanism} Let $f:\D^n\to\re^p$ be a vector valued function. For a given data set $D$, the objective is to output an approximation to $f(D)$ while preserving differential privacy. Let $\eta=\max\limits_{D,D' \text{ s.t. }|D\triangle D'|=2}\ltwo{f(D)-f(D')}$ be the \emph{sensitivity} of the function $f$. Gaussian mechanism refers to the following algorithm: Output $f(D)+\mathcal{N}\left(0,\I_p\frac{4\eta^2\log(1/\delta)}{\epsilon^2}\right)$. One can show that the above algorithm is $(\epsilon,\delta)$-differentially private. (See \cite[Lemma 4]{nikolov2013geometry} for a proof.) Using the proof technique of \cite[Lemma 4]{nikolov2013geometry} one can easily show that the theorem also holds for $(\epsilon,\delta)$-measure stability at any given data set $D\in\D^n$, with $\eta=\max\limits_{D',|D\triangle D'|=2}\ltwo{f(D)-f(D')}$.
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout_nips"
%%% End:


==> tex/appNonRobust.tex <==
\section{Proof of Theorem~\ref{thm:boundDropComplex}}\label{app:nonRobust}
\begin{proof}
Let $e=g-f$ be the error polynomial for the approximation $g$ and let $\hat e=\hat g -f$ be the error polynomial for the approximation $\hat g$. We have the following identity. Here $\Delta g=\hat g-g$, and the last step in\eqref{eqn:errorIdent} is for notational purposes.
\begin{align}
&\E\limits_{x}\left[|\hat g(x)-f(x)|^2\right]=\E\limits_{x}\left[| g(x)+\Delta g(x)-f(x)|^2\right]\nonumber\\
&=\E\limits_{x}\left[| g(x)-f(x)|^2\right]+\E\limits_{x}\left[|\Delta g(x)|^2\right]\nonumber\\&\hspace*{1.5in}+2\E\limits_{x}\left[\left((g(\bar x)-f(\bar x))\Delta g(x)\right)\right]\nonumber\\
&\Leftrightarrow \E\limits_{x}\left[|\hat e(x)|^2\right]-\E\limits_{x}\left[|e(x)|^2\right]=\E\limits_{x}\left[|\Delta g(x)|^2\right]\nonumber\\&\hspace*{1.5in}+2\E\limits_{x}\left[\left((g( x)-f( x))\Delta g(x)\right)\right]\nonumber\\
&\Leftrightarrow \ld{\hat e}^2-\ld{e}^2=\underbrace{\ld{\Delta g}^2}_A+\underbrace{2\ipd{\Delta g}{g-f}}_B
\label{eqn:errorIdent}
\end{align}
We first analyze the term $B$. Notice that one can equivalently write the polynomial $g-f$ as $\sum\limits_{i=1}^m\alpha_i\mu_i g_i$, where $\mu_i\sim_{\sf unif}\{-1,1\}$. For any $x\in\X$, the following in \eqref{eq:zeroMean} is true.
\begin{equation}
\E\limits_{\mu}\left[\sum\limits_{i\in[m]}\alpha_i \mu_i \ipd{g_i}{g-f}\right]=0.
\label{eq:zeroMean}
\end{equation}
In order to lower bound $B$ in \eqref{eqn:errorIdent}, along with \eqref{eq:zeroMean} we now need to lower bound the variance of $B$, i.e., lower bound the random variable $Z=\ipd{\Delta g}{g-f}^2$. By the randomness of $\mu_i$'s we have $\E\limits_{\mu}[Z]=\sum\limits_{i=1}^m\alpha_i^2\ipd{g_i}{g-f}^2$. Also by \eqref{eq:lbErrV}, we have $\E\limits_\mu[Z^2]\leq 2\left(\sum_{i}\alpha_i^2\ipd{g_i}{g-f}^2\right)^2$. Using standard Payley-Zigmund anti-concentration inequality, we have $\Pr[Z\geq\E[Z]/2]\geq\frac{(\E[Z]^2)}{4\E[Z^2]}$. Plugging in the bounds on $Z$ from above we have $\Pr[Z\geq\E[Z]/2]\geq 1/4$.

\begin{align}
\E\limits_{\mu}[Z^2]&=\E\limits_{\mu}\left[\left(\sum\limits_{i=1}^m\alpha_i\mu_i\ipd{g_i}{g-f}\right)^4\right]\nonumber\\
&=\E\limits_{\mu}\left[\sum\limits_{i,j,k,\ell}(\alpha_i\alpha_j\alpha_k\alpha_\ell)\cdot(\mu_i\mu_j\mu_k\mu_\ell)\ipd{g_i}{g-f}\ipd{g_j}{g-f}\ipd{g_k}{g-f}\ipd{g_\ell}{g-f}\right]\nonumber\\
&\leq 2\E\limits_{\mu}\left[\left(\sum_{i,j}\alpha_i\alpha_j\mu_i\mu_j\ipd{g_i}{g-f}\ipd{g_j}{g-f}\right)^2\right]\nonumber\\
&=2\sum_{i,j}\alpha_i^2\alpha_j^2\ipd{g_i}{g-f}^2\ipd{g_j}{g-f}^2\leq 2\left(\sum_{i}\alpha_i^2\ipd{g_i}{g-f}^2\right)^2
\label{eq:lbErrV}
\end{align}

In \eqref{eq:lb1s} we lower bound $\E\limits_{\mu}[Z]$ as follows. In \eqref{eq:lb1s} we have used the assumption that $\ld{g}^2\geq\ld{f}^2$. Using the fact in \eqref{eq:zeroMean} and \eqref{eq:lb1s}, it follows that with probability at least $1/4$, we have $2\ipd{\Delta g}{g-f}\geq -\frac{\alpha_{\min}}{2\sqrt m}\ld{g-f}^2$.
\begin{align}
\E\limits_{\mu}[Z]&=\sum\limits_{i=1}^m\alpha_i\ipd{\alpha_i g_i}{g-f}^2\geq\frac{\alpha_{\min}}{m}\left(\sum\limits_{i=1} ^m\left|\ipd{\alpha_i g_i}{g-f}\right|\right)^2\nonumber\\
&\geq\frac{\alpha_{\min}}{m}\ipd{g}{g-f}^2=\frac{\alpha_{\min}}{4m}\ld{g-f}^4
\label{eq:lb1s}
\end{align}
Now we focus on the term $A$ in \eqref{eqn:errorIdent} and provide an upper bound. We have $\E\limits_{\mu}\left[\ld{\Delta g}^2\right]=\sum\limits_{i=1}^m\alpha_i^2\ld{g_i}^2$. Using the bounds on the terms $A$ and $B$ one can conclude that if $\ld{g-f}^2\geq\frac{\ltwo{\alpha}^2\max\limits_{i\in [m]}\ld{g_i}^2\sqrt m}{16\sqrt{\alpha_{\min}}}$, then with probability at least $1/8$, $\ld{\hat g-f}^2\leq\left(1-\frac{\sqrt{\alpha_{\min}}}{4\sqrt m}\right)\ld{g-f}^2$. This completes the proof.
\end{proof}


==> tex/appdropStabBackup.tex <==
\section{Missing proofs from section \ref{sec:stabDropout} (Stability of dropout)}
\label{app:dropStab}

\subsection{Missing proof of theorem \ref{thm:modelSGD} (Stability of dropout for SGD)}
\label{app:modelSGD}

\begin{proof}
We will follow the notation from Section \ref{sec:SGDDrop} for convenience. Recall that\\ $J(\theta;D)=\frac{1}{n}\sum\limits_{i=1}^n\E\limits_{b\sim\{0,1\}^p}\left[\ell(2\ip{x_i*b}{\theta};y_i)\right]$ and $\ell_t(\theta)=\ell(2\ip{\hat x_t*b_t}{\theta};\hat y_i)$, where $x_t,y_t$ and $b_t$ are the parameters used in the $t$-th iterate. By the same argument as in \eqref{eq:akjhd123} we have that $J(\theta;D)$ and $J(\theta;D')$ are $\Lambda$-strongly convex, where $D'$ is any neighboring data set of $D$.

Let $\theta_T(D)$ and $\theta_T(D')$ the outputs of SGD on data sets $D$ and $D'$. Similarly, let $\theta^\dagger(D)=\arg\min\limits_{\theta\in\C} J(\theta;D)$ and $\theta^\dagger(D')$ be defined analogously. Using an immediate variant of  Theorem \ref{thm:stocGradConv} we conclude that for $\theta_T$ (i.e., the $\theta$ obtained after running the SGD algorithm for $T$), $\E[J(\theta_T(D);D)-J(\theta^\dagger(D);D)]=O\left(\frac{(GB)^2\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{\Lambda T}\right)$ .
By the $\Lambda$-strong convexity of $J(\theta;D)$ and Jennsen's inequality, we have the following:
\begin{equation}
\E\left[\ltwo{\theta_T(D)-\theta^\dagger(D)}\right]=O\left(\frac{GB}{\Lambda}\left(\sqrt{\frac{\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{T}}\right)\right).
\label{eq:09ad}
\end{equation}
The same bound holds for the data set $D'$ too. In order to complete the stability argument, we show that on a neighboring data set $D'$, $\theta^\dagger(D)$ does not change too much in $L_2$-norm. W.l.o.g. assume that $D$ and $D'$ differ in the $n$-th data entry. Therefore, by strong convexity and the property of the minimizers $\theta^\dagger(D)$ and $\theta^\dagger(D')$, we have the following. For brevity we represent  $f(\theta;x,y)=\frac{1}{n}\E\limits_{b\sim\{0,1\}^p}\left[\ell(2\ip{x*b}{\theta};y)\right]$.
\begin{align}
&J(\theta^\dagger(D');D)\geq J(\theta^\dagger(D);D)+\frac{\Lambda}{2}\ltwo{\theta^\dagger(D')-\theta^\dagger(D)}^2\nonumber\\
&\Leftrightarrow J(\theta^\dagger(D');D)+f(\theta^\dagger(D');y_n',x_n')-(J(\theta^\dagger(D);D)+f(\theta^\dagger(D);y_n',x_n'))\geq\frac{\Lambda}{2}\ltwo{\theta^\dagger(D')-\theta^\dagger(D)}^2\nonumber\\
&+\left(f(\theta^\dagger(D');y_n',x_n')-f(\theta^\dagger(D);y_n',x_n')\right)\nonumber\\
&\Leftrightarrow J(\theta^\dagger(D');D')-J(\theta^\dagger(D);D')\geq\frac{\Lambda}{2}\ltwo{\theta^\dagger(D')-\theta^\dagger(D)}^2+\left(f(\theta^\dagger(D');y_n',x_n')-f(\theta^\dagger(D);y_n',x_n')\right)\nonumber\\
&\Leftrightarrow\left(f(\theta^\dagger(D);y_n',x_n')-f(\theta^\dagger(D');y_n',x_n')\right)\geq\frac{\Lambda}{2}\ltwo{\theta^\dagger(D')-\theta^\dagger(D)}^2\nonumber\\
&\Rightarrow\ltwo{\theta^\dagger(D')-\theta^\dagger(D)}=O\left(\frac{GB}{n\Lambda}\right).
\label{eq:loq123}
\end{align}
Now notice that Theorem \ref{thm:stocGradConv} is true for any data set. Therefore combining \eqref{eq:loq123} and \eqref{eq:09ad}, we have
$\E\left[\ltwo{\theta_T(D)-\theta_T(D')}\right]=O\left(\frac{GB}{\Lambda}\left(\sqrt{\frac{\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{T}}+\frac{1}{n}\right)\right)$.

This completes the proof.
\end{proof}

\subsection{Stability of dropout for empirical risk minimization}
\label{app:stabERM}

\begin{thm}[Model stability of the ERM formulation]
Let $\C\subseteq\re^p$ be a fixed convex set and let Assumption \ref{assump:normDat} be true for the data domain $\D$ and the loss $\ell$.
Let $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ be $n$ samples from $\D$ and let $\{b_1,\cdots,b_n\}$ be the corresponding dropout vectors in \eqref{eq:dropout}. Let $\Lambda=\frac{1}{n}\min\limits_{k\in[n]}\min\limits_{j\in[p]}\sum\limits_{i=1,i\neq k}^n x_i(j)^2$. Assuming $\Lambda=\omega(({\sf poly}\log n)/n)$ and the dimensions $p=O({\sf poly}(n))$, it follows that the ERM with dropout is $\epsilon$-model stable, where $\epsilon=O\left(\frac{GB}{\Lambda n}\right)$. Here $G$ and $B$ are parameters from Assumption \ref{assump:normDat}.
\label{thm:stabERM}
\end{thm}

\begin{proof}
Let $\hJ(\theta;D)=\frac{1}{n}\sum\limits_{i=1}^n \ell(2\ip{x_i * b_i}{\theta};y_i)$ and ${\widehat \theta}(D)=\arg\min\limits_{\theta\in\C}\hJ(\theta;D)$ for the ease of notation. We have
\begin{align*}\nabla^2_\theta {\hJ}(\theta;D)&=\frac{4}{n}\sum\limits_{i=1}^n\left[\frac{\partial^2 \ell(2\ip{x_i*b_i}{\theta};y_i)}{\partial \ip{2x_i*b_i}{\theta}^2}(x_i*b_i)(x_i*b_i)^T\right] \nonumber\\
&\succeq \frac{4}{n}\sum\limits_{i=1}^n\left[(x_i*b_i)(x_i*b_i)^T\right].
\end{align*}
From the above expression, one can observe that $\E\limits_{b_1,\cdots,b_n}\left[\grad^2 J(\theta;D)\right]=\frac{1}{n}\sum\limits_{i=1}^n\left(x_i x_i^T+\diag(x_i x_i^T)\right)$.
Therefore, $\lambda_{min}\left(\E\limits_{b_1,\cdots,b_n}\left[\grad^2 J(\theta;D)\right]\right)\geq\Lambda$.
Additionally, for any $i\in[n]$, $\frac{4}{n}\lambda_{max}(x_i x_i^T)\leq\frac{4B^2}{n}$. Therefore by Matrix Chernoff bound, over the randomness of $b_1,\cdots,b_n$, we have
\begin{equation}
\Pr\left[\lambda_{min}\left(\grad^2 J(\theta;D)\right)\leq \frac{\Lambda}{2}\right]\leq p\cdot \exp\left(-\Omega(n\Lambda/B^2)\right).
\label{eq:cher12}
\end{equation}
The same bound in \eqref{eq:cher12} holds for any neighboring data set $D'$. W.l.o.g. assume that $D$ and $D'$ differ in the $n$-th data entry. Therefore, by strong convexity and the property of the minimizers $\theta^\dagger(D)$ and $\theta^\dagger(D')$, we have the following w.p. at least $1-2p\cdot \exp\left(-\Omega(n\Lambda/B^2)\right)$. For brevity we represent  $f(\theta;x_i,y_i)=\frac{1}{n}\ell(2\ip{x_i*b_i}{\theta};y_i)$.
\begin{align}
&\hJ({\widehat \theta}(D');D)\geq \hJ({\widehat \theta}(D);D)+\frac{\Lambda}{2}\ltwo{{\widehat \theta}(D')-{\widehat \theta}(D)}^2\nonumber\\
&\Leftrightarrow \hJ({\widehat \theta}(D');D)+f({\widehat \theta}(D');y_n',x_n')-(\hJ({\widehat \theta}(D);D)+f({\widehat \theta}(D);y_n',x_n'))\geq\frac{\Lambda}{2}\ltwo{{\widehat \theta}(D')-{\widehat \theta}(D)}^2\nonumber\\
&+\left(f({\widehat \theta}(D');y_n',x_n')-f({\widehat \theta}(D);y_n',x_n')\right)\nonumber\\
&\Leftrightarrow \hJ({\widehat \theta}(D');D')-\hJ({\widehat \theta}(D);D')\geq\frac{\Lambda}{2}\ltwo{{\widehat \theta}(D')-{\widehat \theta}(D)}^2+\left(f({\widehat \theta}(D');y_n',x_n')-f({\widehat \theta}(D);y_n',x_n')\right)\nonumber\\
&\Leftrightarrow\left(f({\widehat \theta}(D);y_n',x_n')-f({\widehat \theta}(D');y_n',x_n')\right)\geq\frac{\Lambda}{2}\ltwo{{\widehat \theta}(D')-{\widehat \theta}(D)}^2\nonumber\\
&\Rightarrow\ltwo{{\widehat \theta}(D')-{\widehat \theta}(D)}=O\left(\frac{GB}{n\Lambda}\right).
\label{eq:loq123as}
\end{align}
Therefore, by \eqref{eq:cher12} and \eqref{eq:loq123as}, as long as $p=O({\sf poly}(n))$, we have the required bound.
\end{proof}

\subsection{High-probability model stability of dropout}
\label{app:highProbModStab}

\begin{thm}[High probability model stability of SGD]
Let $k=\log(1/\delta)$ be the number of independent runs of stochastic gradient descent. Following the notation of Theorem \ref{thm:modelSGD}, with probability at least $1-\delta$  over the randomness of the algorithm, we have the following.
$$\ltwo{\theta^{(j^*)}_T(D)-\theta^{(j^*)}_T(D')}=O\left(\frac{GB\sqrt{\log(1/\delta)}}{\Lambda}\left(\sqrt{\frac{\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{T}}+\frac{1}{n}\right)\right).$$
Here $D'$ is any neighboring data set of $D$.
\label{thm:highProbModStab}
\end{thm}

\begin{proof}
Let $\theta^\dagger=\arg\min\limits_{\theta\in\C}J(\theta;D)$. Notice that by Markov's inequality and the bound from Theorem \ref{thm:stocGradConv} one can conclude that w.p. at least $1/2$, for a given $j\in[k]$, $J(\theta^{(j)}_T;D)-J(\theta^\dagger;D)=O\left(\frac{(GB)^2\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{\Lambda T}\right)$. For $k=\log(1/\delta)$ independent runs of the stochastic gradient descent, it follows that with probability at least $1-\delta$, $$J(\theta^{(j^*)}_T;D)-J(\theta^\dagger;D)=O\left(\frac{(GB)^2\log T\log(1/\delta)\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{\Lambda T}\right).$$ Now following the rest of the argument exactly as Theorem \ref{thm:modelSGD}, we get the required bound.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout_nips"
%%% End:


==> tex/convDropDiff.tex <==
\subsection{Converting dropout optimization to a differentially private algorithm}\label{sec:convDiffPrivate}
Notice that all of our stability guarantees in Section \ref{sec:stabDropout} are independent of the data distribution $\tau(D)$. This has direct implications for differential privacy. We show that using the \emph{propose-test-release} (PTR) framework \cite{DL09,STLasso13}, the dropout heuristic provides a \emph{differentially private} algorithm.

\begin{defn}[$(\epsilon,\delta)$-differential privacy \cite{DMNS06,ODO}]\label{def:diffPrivacy}
	For any pairs of  neighboring data sets $D,D'\in\D^n$ differing in exactly one entry, an algorithm $\A$ is $(\epsilon,\delta)$-differentially private if for all measurable sets $S$ in the range space of $\A$ the following holds:
	$$\Pr[\A(\D)\in S]\leq e^\epsilon\Pr[\A(\D')\in S]+\delta.$$
\end{defn}
The $(\epsilon,\delta)$-measure stability guarantees from Sections \ref{sec:linLoss} and \ref{sec:dropoutQuadratic} can be interpreted as follows. For a given algorithm $\A$ and a level of accuracy $\sigma$ (or a bound on the extra randomness for measure stability), there exists a deterministic function $g_{\A,\sigma}:\D^n\to\re$. If $g_{\A,\sigma}(D)$ exceeds a threshold $\zeta$, then $\A(D)$ is $(\epsilon,\delta)$-measure stable at $D$. We drop the dependency of $g$ on $\A$ and $\sigma$ in the sequel.

As an example, consider the measure stable variant of dropout in Section \ref{sec:dropoutQuadratic}. Recall that to achieve measure stability, we introduced Gaussian perturbations to the model. If we require that the standard deviation of the noise added is bounded by $\sigma$ (corresponding to a given level of accuracy) and we expect $(\epsilon,\delta)$-differential privacy, then it suffices for $\Lambda$ (defined in Theorem \ref{thm:modelSGD}) to be at least $\max\left\{O\left(\frac{GB}{\epsilon\sigma}\left(\sqrt{\log T}/T+\frac{1}{n}\right)\right),\frac{\Delta_1}{2}\right\}$, and for $g(D)=\Lambda$.

For the settings in this paper, $g$ has bounded sensitivity (i.e., for any pair of neighboring data sets $D$ and $D'$, $|g(D)-g(D')|\leq \eta$). Notice that in our above example, with $g(D)=\Lambda$, the sensitivity of $g$ is $\eta=\frac{B}{n}$ (where $B$ upper bounds the $L_2$ norm of any feature vector $x$). For differential privacy, bounded sensitivity is essential. The following two-stage algorithm ensures $(\epsilon,\delta)$-differential privacy for dropout.
\begin{enumerate}
    \item \textbf{Noisy estimate of $g$:} $\widehat g\leftarrow g(D)+{\sf Lap}(\eta/\epsilon)$, where ${\sf Lap}(\lambda)$ is drawn from $\frac{1}{2\lambda}e^{-|x|/\lambda}$.
    \item \textbf{Test for safety:} If $\widehat g>\zeta+\left(\eta\cdot\log(1/\delta)/\epsilon\right)$, then execute dropout heuristic, otherwise fail.
\end{enumerate}
One can show using tail bounds that if $g(D)>\zeta+\left(\eta\cdot\log(1/\delta)/\epsilon\right)$, then w.p.~at least $1-\delta$, the above algorithm will output the execution of the dropout heuristic exactly.


\mypar{Optimality of error} Regularized private risk minimization is a well-studied area \cite{CM08,DL09,CMS11,JKT12,KST12,DuchiJW13,song2013stochastic,jain2014near,BST}. Here we provide yet another algorithm for private risk minimization. While the previous algorithms primarily used variants of $L_2$ regularization, we use the dropout regularization for the privacy guarantee. Conditioned on the PTR test passing, the utility of this algorithm follows from the learning bounds obtained for the measure stable version of dropout which depends on the noise level $\sigma$. While the bounds are tight in general \cite{BST} and there exists other algorithms achieving the same bounds \cite{BST,jain2014near}, since dropout has been often shown to outperform vanilla regularization schemes, it might be advantageous to use dropout learning even in the context of differential privacy. (See Section \ref{sec:experiments} for more discussions.)  

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout_nips"
%%% End:


==> tex/dropoutGenBackup.tex <==
\section{Dropout as a Regularizer and its Excess Risk Analysis}
\label{sec:dropoutGen}
In this section, we show that dropout when applied to the ERM formulation acts as a regularizer and hence removes need for explicit regularization. In particular, for the special case of least squares linear regression, dropout regularization is similar to the $L_2$ regularization. Based on this observation, we provide explicit fast rates for the excess risk.

For simplicity of the exposition, we modify ERM formulation to incorporate dropout perturbation as part of the optimization problem itself. We then observe that for GLM with strongly convex loss function, dropout acts as a regularizer and then provide the excess risk rates.
%In this section we state the dropout heuristic for the case of generalized linear models, and provide the risk bounds for the specific case of linear regression.
\subsection{An Empirical Risk Minimization (ERM) Formulation}
\label{sec:ERM}
For a given loss function $\ell$ and the convex set $\C$ as defined as in Section \ref{sec:probDef}, and a data set $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$, dropout heuristic refers to optimizing the following objective function:
\begin{equation}
\nptheta=\arg\min\limits_{\theta\in\C}\frac{1}{n}\sum\limits_{i=1}^n \ell(2\ip{x_i * b_i}{\theta};y_i)
\label{eq:dropout}
\end{equation}
Here each $b_i$ is an i.i.d. sample drawn uniformly from $\{0,1\}^p$, and the operator $*$ refers to the Hadamard product. We assume that the loss function $\ell(u, y):\R^2\rightarrow \R$ is strongly convex in $u$. For example, in the case of linear regression, the loss function $\ell(2\ip{x}{\theta};y)$ is $(y-2\ip{x}{\theta})^2$.

We would like to stress this formulation of dropout is for intuition only. In Section \ref{sec:SGDDrop}, we discuss the classic version of dropout using stochastic gradient descent.

\begin{lem}
  Let $b$ be drawn uniformly from $\{0,1\}^p$. Recall that, the expected population risk is given by:
$${\sf Risk}(\theta)=\E_{(x,y)\sim\tau(\D), b}[\ell(2\ip{x*b}{\theta};y)].$$
Let $\ell(u, y)$ be a $\alpha$-strongly convex function in $u$ for all $y$. Then, the expected population risk (given above) is $\alpha \cdot \lambda_{min}$ strongly convex w.r.t. $\theta$, where $\lambda_{min}=\min_{j}\E_{(x,y)\sim\tau(\D)}[x(j)^2]$ and $x(j)$ is the $j$-th coordinate of $x$. \label{lem:risk_sc}
\end{lem}
\begin{proof}
Now,
  \begin{align*}\nabla^2_\theta {\sf Risk}(\theta)&=\E_{(x,y)\sim\tau(\D)}\left[\E_{b}\left[4\frac{\partial^2 \ell(\ip{x*b}{\theta};y)}{\partial \ip{x*b}{\theta}^2}(x*b)(x*b)^T\right]\right] \nonumber\\
&\succeq 4\alpha\E_{(x,y)\sim\tau(\D)}\left[\frac{1}{4}\diag(xx^T)+\frac{1}{4}xx^T\right]\succeq \alpha \lambda_{min},\end{align*}
where second to last inequality follows by strong convexity of $\ell$ and by using the fact that $b$ is sampled uniformly from $\{0, 1\}^{p}$.
\end{proof}

\begin{corollary}
  Let $b$ be drawn uniformly from $\{0,1\}^p$ and let $\ell(2\ip{x}{\theta};y)$ be the least squares loss function, i.e., $\ell(2\ip{x}{\theta};y)=(2\ip{x}{\theta}-y)^2$. Then, \begin{equation}{\sf Risk}(\theta)=\E\limits_{(x,y)\sim\tau(\D)}\left[(y-\ip{x}{\theta})^2+\theta^T \diag(\langle x(1)^2,\cdots,x(p)^2\rangle)\theta\right].\label{eq:linearRisk}\end{equation}
\end{corollary}

The above corollary shows that for datasets with normalized features that is where $\E[\sum_j x(j)^2]=1$, the dropout objective based risk function is the same as $L_2$ regularized least squares (in expectation).
Also, note that even for least squares problem where the Hessian is not positive definite (for example, where each $x=\langle 1, 1, \dots 1,\rangle\in \R^{p}$),  dropout objective's expected risk is a $1$-strongly convex function.

Next, we provide excess risk bound for $\nptheta$, the optimal solution to the dropout based ERM (defined in \eqref{eq:dropout}). Our proof technique follows closely the analysis of \cite{sridharan2008fast}, and crucially uses the fact that the analysis of \cite{sridharan2008fast} only requires strong convexity of the ``expected'' loss function. Below we provide the risk bound; detailed proof is provided in the appendix. % only our results do not directly follow from  since the dropout loss function in \eqref{eq:dropout} is not strongly convex. However, as we will see it demonstrates strong convexity property in expectation and that is sufficient for the excess risk bound.

%For linear regression, we compare the generalization ability of the of the minimizer $\nptheta$, with respect to the following risk function
%\begin{equation}
%{\sf Risk}(\theta)=\E\limits_{(x,y)\sim\tau(\D)}\left[(y-\ip{x}{\theta})^2+\theta^T \diag(\langle x(1)^2,\cdots,x(p)^2\rangle)\theta\right].
%\label{eq:linearRisk}
%\end{equation}
%Here the vector $\langle x(1)^2,\cdots,x(p)^2\rangle$ refers to the vector of the squares of the coordinates of $x$, and the operator $\diag(v)$ refers to a $p\times p$ diagonal matrix with the vector $v$ forming the diagonal entries. In the following, we provide the following excess risk bound for $\nptheta$ (defined in \eqref{eq:dropout}). While the proof technique follows closely the analysis of \cite{sridharan2008fast}, but our results do not directly follow from theirs since the dropout loss function in \eqref{eq:dropout} is not strongly convex. However, as we will see it demonstrates strong convexity property in expectation and that is sufficient for the excess risk bound.

\begin{thm}[Dropout generalization bound]
Let the domain of data entries $\D$ be defined such that for any $(x,y)\in\D, \ltwo{x}\leq 1$ and $\ltwo{y}\leq 1$, and let $\C\subseteq\re^p$ be a fixed convex set. Let $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ be $n$ i.i.d. samples drawn from $\tau(\D)$. Let $B=\{b_1,\cdots,b_n\}$ be $n$ i.i.d. vectors drawn uniformly from $\{0,1\}^p$. Let $\nptheta=\arg\min\limits_{\theta\in\C}\frac{1}{n}\sum\limits_{i=1}^n \ell(2\ip{x_i * b_i}{\theta};y_i)$ and let $\rL(\theta)=\E\limits_{(x,y)\sim\tau(\D)}\left[\ell(2\ip{x}{\theta};y)\right]$. Also, let $\ell$ be $1$-strongly convex and $|\frac{\partial \ell(u; y)}{\partial u}|\leq G$.
Then, w.p. $\geq 1-\gamma$ (over the randomness of both $D$ and $B$), we have the following:
$$\E\left[\rL(\nptheta)-\min\limits_{\theta\in\C}\rL(\theta)\right]=O\left(\frac{G^2\log(1/\gamma)}{\Delta n}\right).$$
Here $\Delta=\min\limits_{j\in[p]}{\E\limits_x\left[x(j)^2\right]}$.
\label{thm:dropoutGen}
\end{thm}

\begin{proof}
%In the case of linear regression with dropout, we have the following optimization problem. (Here the notation is same as \eqref{eq:dropout}.)
%\begin{equation}
%\nptheta=\arg\min\limits_{\theta\in\C}\frac{1}{n}\sum\limits_{i=1}^n (y_i-2\ip{x_i * b_i}{\theta})^2
%\label{eq:dropoutLin}
%\end{equation}

%Let $H=\{(x_1*b_1,y_1),\cdots,(x_n*b_n,y_n)\}$ be a data set of  i.i.d. samples drawn from $\tau(\D)\times \{0,1\}^p$, corresponding to the data set $D$ and the noise vectors $b_1,\cdots,b_n$ in \eqref{eq:dropoutLin}. Notice that if we consider the feature vectors to be $x_i*b_i$ for any $i\in[n]$, the optimization problem above is in the generalized linear model (GLM). So, in effect we can borrow tools from the excess risk bound analyses for GLMs present in the literature \cite{SSSS,sridharan2008fast}. For the ease of notation, let $\dL(\theta)=\frac{1}{n}\sum\limits_{i=1}^n (y_i-2\ip{x_i * b_i}{\theta})^2$. In the following claim we relate $\dL$ and $\rL$ (see Theorem \ref{thm:dropoutGen} for the definition).

%\begin{claim}
%The following is true.
%$$\E\limits_H \left[\dL(\theta)\right]=\E\limits_{(x,b,y)}\left[(y-2\ip{x*b}{\theta})^2\right]=\rL(\theta).$$
%\label{cl:1}
%\end{claim}
%\begin{proof}
%The first equality in the above claim follows immediately from the fact that the samples in the data set $H$ are i.i.d. samples. In the following we prove the second equality.

%Corresponding to a given vector $b\in\{0,1\}^p$, let $w\in\{-1,1\}$ be a vector which replaces the zeroes in $b$ with $-1$. For any $x,y\in\re^p$ and $b\in\{0,1\}^p$, one can observe the following.
%\begin{equation}
%(y-2\ip{x*b}{\theta})^2=(y-\ip{x}{\theta})^2+\theta^T\left[(x*w)(x*w)^T\right]\theta-2y\ip{x*w}{\theta}+2\ip{x}{\theta}\ip{x*w}{\theta}
%\label{eq:121}
%\end{equation}
%Taking the expectation over the randomness of $b$ (and correspondingly $w$) we have
%\begin{align}
%\E_b\left[(y-2\ip{x*b}{\theta})^2\right]&=(y-\ip{x}{\theta})^2+\E_w\left[\theta^T\left[(x*w)(x*w)^T\right]\theta\right]\nonumber\\
%&-2\E_w\left[y\ip{x*w}{\theta}-\ip{x}{\theta}\ip{x*w}{\theta}\right]\nonumber\\
%&=(y-\ip{x}{\theta})^2+\theta^T\diag(\langle x(1)^2,\cdots,x(p)^2\rangle)\theta
%\label{eq:122}
%\end{align}
%The last equality follows from the unbiasedness of the random vector $w$. Now taking expectation w.r.t. $(x,y)$ on both sides of \eqref{eq:122} completes the claim.
%\end{proof}
%With above claim in hand, we focus on bounding the following excess risk for $\nptheta$:
%\begin{equation}
%\L(\theta)-\min\limits_{\theta\in\C}\E\limits_{(x,b,y)}\left[(y-2\ip{x*b}{\theta})^2\right]
%\label{eq:1amc}
%\end{equation}
Define $g_\theta$ as: $g_\theta(x,y,b)=\ell(2\ip{x*b}{\theta};y)-\ell(2\ip{x*b}{\theta^*};y)$, where $\theta^*=\arg\min\limits_{\theta\in\C}\E\limits_{(x,b,y)}\left[\ell(2\ip{x*b}{\theta};y)\right]$. Also, let $\mathcal{G}_\theta=\{g_\theta:\theta\in\C\}$.
% Let $f(\theta;x,y,b)=\ell(2\ip{x*b}{\theta};y)$ and $\theta^*=\arg\min\limits_{\theta\in\C}\E\limits_{(x,b,y)}\left[f(\theta;x,y,b)\right]$.
%For each $\theta$, let $g_\theta(x,y,b)=f(\theta;x,y,b)-f(\theta^*;x,y,b)$ and $\mathcal{G}_\theta=\{g_\theta:\theta\in\C\}$.
Following the technique of \cite{sridharan2008fast}, we will now scale each of the $g_\theta$'s such that the ones which have higher expected value over $(x,y,b)$ have exponentially smaller weight. This helps us obtain a more fine-grained bound on the Rademacher complexity, which will be apparent below.

Let $\mathcal{G}_a=\left\{g_\theta^a=\frac{g_\theta}{4^{k_a(\theta)}}:\theta\in\C,k_a(\theta)=\min\left\{k'\in\mathbb{Z}^+:\E\limits_{(x,y,b)}[g_\theta]\leq a4^{k'}\right\}\right\}$. Using standard Rademacher complexity bounds \cite[Theorem 5]{bousquet2004introduction}, for any $\theta\in\C$, the following holds (w.p. $\geq 1-\delta$ over the randomness in selection of dataset $H$): %we have the following  with probability $1-\gamma$ over the randomness in the selection of the dataset $H$:
\begin{equation}
\sup\limits_{q\in\mathcal{G}_a}\left[\E\limits_{(x,y,b)}\left[q(x,y,b)\right]-\frac{1}{n}\sum\limits_{i=1}^n q(x_i,y_i,b_i)\right]\leq 2\mathcal{R}(\mathcal{G}_a)+\left(\sup\limits_{q\in\mathcal{G}_a,(x,y,b)}|q(x,y,b)|\right)\sqrt\frac{\log(1/\gamma)}{2n}
\label{eq:l123}
\end{equation}
Here $\mathcal{R}$ refers to the Rademacher complexity of the hypothesis class. In the following we will bound each of the term in the right hand side of \eqref{eq:l123}.

\begin{lem}
Let $\Delta=\min\limits_{j\in[p]}{\E\limits_x\left[x(j)^2\right]}$, where $x(j)$ refers to the $j$-th coordinate of $x$. The following is true.
$$\sup\limits_{q\in\mathcal{G}_a,(x,y,b)}|q(x,y,b)|\leq 2 G\sqrt\frac{2a}{\Delta}.$$
\label{lem:121}
\end{lem}
\begin{proof}
By the definition of the bound on the domain of $x$ and assumption on $\ell$, we have $\ltwo{\grad_\theta \ell(2\ip{x*b}{\theta};y)}\leq 2G$. Therefore $\forall\theta\in\C, q\in\mathcal{G}_a, (x,y)\in\D, b\in\{0,1\}^p$, we have the following.
\begin{equation}
|q(x,y,b)|\leq\frac{|g_\theta(x,y,b)|}{4^{k_a(\theta)}}\leq \frac{2G\ltwo{\theta-\theta^*}}{4^{k_a(\theta)}}.
\label{eq:1223a}
\end{equation}
In the following we now bound $\ltwo{\theta-\theta^*}$. Using Lemma~\ref{lem:risk_sc}, $\E\limits_{x, y, b}[ \ell(2\ip{x*b}{\theta};y)]$ is strongly convex and hence using optimality of $\theta^*$, we have: %Notice that $F(\theta)=\E\limits_{x,y,b}[f(\theta;x,y,b)]$ is $\Delta=\min\limits_{j\in[p]}{\E\limits_x\left[x(j)^2\right]}$-strongly convex, where $x(j)$ refers to the $j$-th coordinate of $x$. This observation follows immediately from \eqref{eq:122}. Therefore by strong convexity property, we have the following.
\begin{equation}
\ltwo{\theta-\theta^*}\leq\sqrt{\frac{2}{\Delta}\E\limits_{x,y,b}[g_\theta(x,y,b)]}\leq \sqrt{\frac{2a\cdot 4^{k_a(\theta)}}{\Delta}},
\label{eq:12a}
\end{equation}
where the last equations follows using definition of $k_a(\theta)$. %By the definition of $k(\theta)$, it implies that $\E\limits_{x,y,b}[g_\theta(x,y,b)]\leq a 4^{k(\theta)}$. Therefore from \eqref{eq:12a} we have the following.%
%\begin{equation}
%\ltwo{\theta-\theta^*}\leq \sqrt{\frac{2a\cdot 4^{k(\theta)}}{\Delta}}\leq \sqrt{\frac{2a\cdot 16^{k(\theta)}}{\Delta}}.
%\label{eq:12b}
%\end{equation}
%Plugging \eqref{eq:12b} in \eqref{eq:1223a} gives the required bound.
\end{proof}
Now, directly using \cite[Lemma 7]{sridharan2008fast}, we can bound the Rademacher complexity in \eqref{eq:l123} by $\mathcal{R}(\mathcal{G}_a)\leq 4\sqrt\frac{128a}{\Delta n}$. Therefore we can bound \ref{eq:l123} as follows.
\begin{equation}
\sup\limits_{q\in\mathcal{G}_a}\left[\E\limits_{(x,y,b)}\left[q(x,y,b)\right]-\frac{1}{n}\sum\limits_{i=1}^n q(x_i,y_i,b_i)\right]=O\left(G\sqrt\frac{a\log(1/\gamma)}{\Delta n}\right).
\label{eq:l123a}
\end{equation}
Now notice that for any $a>0$, w.p. at least $1-\gamma$ we have the following from \eqref{eq:l123a}.
\begin{align}
\E\limits_{x,y,b}\left[g_\theta(x,y,b)\right]-\frac{1}{n}\sum\limits_{i=1}^n g_\theta (x_i,y_i,b_i)&=4^{k_a(\theta)}\left[\E\limits_{x,y,b}\left[g^a_\theta(x,y,b)\right]-\frac{1}{n}\sum\limits_{i=1}^n g^a_\theta (x_i,y_i,b_i)\right]\nonumber\\
&=4^{k_a(\theta)}O\left(G\sqrt\frac{a\log(1/\gamma)}{\Delta n}\right).
\label{eq:al123}
\end{align}
When ${k_a(\theta)}=0$, \eqref{eq:al123} implies the following.
\begin{equation}
\E\limits_{x,y,b}\left[g_\theta(x,y,b)\right]-\frac{1}{n}\sum\limits_{i=1}^n g_\theta (x_i,y_i,b_i)=O\left(G\sqrt\frac{a\log(1/\gamma)}{\Delta n}\right).
\label{eq:ah12}
\end{equation}
When $k_a(\theta)>0$, one has $4^{k_a(\theta)-1}a<\E\limits_{x,y,b}\left[g_\theta(x,y,b)\right]$. Substituting this in \eqref{eq:al123} and by rearranging the terms, we have the following. Here $M=\xi G\sqrt\frac{a\log(1/\gamma)}{\Delta n}$ for some constant $\xi>0$.
\begin{equation}
\E\limits_{x,y,b}\left[g_\theta(x,y,b)\right]\leq\frac{1}{1-4M/a}\left[\frac{1}{n}\sum\limits_{i=1}^n g_\theta (x_i,y_i,b_i)\right].
\label{eq:op123}
\end{equation}
Setting $a=8M$, and combining \eqref{eq:op123} and \eqref{eq:ah12} for the cases $k_a(\theta)=0$ and $k_a(\theta)>0$ completes the proof.
\end{proof}

\subsection{Dropout with Stochastic Gradient Descent}
\label{sec:SGDDrop}

Given a data set $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ i.i.d. from $\tau(\D)$, a loss function $\ell$ (defined in Section \ref{sec:probDef}) and a fixed convex set $\C$, the dropout stochastic gradient descent (SGD) proceeds as follows. Here $\eta_t$ is the learning rate to be fixed later.

\begin{enumerate}
    \item Pick a uniformly random vector $b_t$ from $\{0,1\}^n$ and a data point $(x_t,y_t)$ uniformly with replacement from $D$.
    \item $\theta_{t+1}\leftarrow\proj_\C\left(\theta_t+4\eta_t x_t*b_t(y_t-2\ip{x_t*b_t}{\theta_t})\right)$.
\end{enumerate}

For linear regression, we compare the generalization ability of the of the minimizer $\theta_T$ (i.e., the vector obtained after running the SGD for $T$ steps) with respect to the risk function defined in \eqref{eq:linearRisk}.

\begin{thm}[Dropout generalization bound for SGD]
Let the domain of data entries $\D$ be defined such that for any $(x,y)\in\D, \ltwo{x}\leq 1$ and $\ltwo{y}\leq 1$, and let $\C\subseteq\re^p$ be a fixed convex set. Let $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ be $n$ i.i.d. samples drawn from $\tau(\D)$. Let $\rL(\theta)=\E\limits_{(x,y)\sim\tau(\D)}\left[(y-\ip{x}{\theta})^2+\theta^T \diag(\langle x(1)^2,\cdots,x(p)^2\rangle)\theta\right]$.
Then over the randomness the SGD algorithm and the distribution $\tau(\D)$, we have the following when the learning rate $\eta_t=\frac{1}{\Delta_1 t}$.
$$\E\left[\rL(\theta_T)-\min\limits_{\theta\in\C}\rL(\theta)\right]=O\left(\frac{\ltwo{\C}^2\log T}{\Delta_1 T}+\frac{\ltwo{\C}^4\log n}{\Delta n}\right).$$
Here $\Delta=\min\limits_{j\in[p]}{\E\limits_x\left[x(j)^2\right]}$ and $\Delta_1=\min\limits_{j\in[p]}\frac{1}{n}\sum\limits_{i=1}^n x_i(p)^2$.
\label{thm:dropoutGenSGD}
\end{thm}
\begin{proof}
Let
\begin{equation}
J(\theta;D)=\frac{1}{n}\sum\limits_{i=1}^n(y_i-\ip{x_i}{\theta})^2+\frac{1}{n}\theta^T\diag(\langle \sum\limits_{i=1}^n x_i(1)^2,\cdots,\sum\limits_{i=1}^n x_i(p)^2\rangle)\theta.
\label{eq:J123}
\end{equation}
Let $\ell_t(\theta)=(y_t-\ip{x_t*b_t}{\theta})^2$ for the ease of notation, where $x_t,y_t$ and $b_t$ are the parameters used in the $t$-th iterate. Over the randomness of the SGD algorithm, we have the following. The proof follows from the gradient version of Claim \ref{cl:1}.
\begin{equation}
\E[\grad \ell_t(\theta)]=\grad J(\theta;D).
\label{eq:gradF}
\end{equation}
Additionally, notice that $J(\theta;D)$ is $\Delta_1$-strongly convex. Using Theorem \ref{thm:stocGradConv} we obtain the bound in \eqref{eq:ambc1321} (over the randomness of the SGD algorithm). Notice that in the context of this paper, $G^2=O(\ltwo{\C}^2)$.

\begin{equation}
\E\left[J(\theta_T;D)-\min\limits_{\theta\in\C} J(\theta;D)\right]=O\left(\frac{\ltwo{\C}^2\log T}{\Delta_1 T}\right).
\label{eq:ambc1321}
\end{equation}

\begin{thm}[Convergence of expected stochastic gradient descent \cite{Ishamir13}]
Suppose $\rL(\theta)$ is a is $\Gamma$-strongly convex function, and let the stochastic gradient descent algorithm be $\theta_{t+1}=\proj_\C(\theta_t-\eta_t\grad \ell_t(\theta))$ such that $\E[\grad\ell_t(\theta)]=\grad J(\theta)$ for all $\theta\in\C$. Additionally, assume that $\E[\ltwo{\grad{\ell_t(\theta_t)}}^2]\leq G^2$ for all $t$. If the learning rate $\eta_t=1/(\Delta_1 t)$, then for any $T>1$ the following is true.
$$\E\left[J(\theta)-\min\limits_{\theta\in\C}J(\theta)\right]=O\left(\frac{G^2\log T}{\Delta_1 T}\right).$$
All the expectations are over the randomness of the stochastic gradient descent algorithm.
\label{thm:stocGradConv}
\end{thm}
Now in the following we state a variant of \cite[Theorem 1]{sridharan2008fast}. The proof of this variant is exactly the same as \cite[Theorem 1]{sridharan2008fast}.

\begin{thm}[Fast convergence for strongly convex objective \cite{sridharan2008fast}]
Over the randomness of the data distribution $\tau(\D)$, for all $\theta\in\C$, the following is true w.p. $\geq 1- \gamma$.
$$\rL(\theta)-\min\limits_{\theta\in\C}\rL(\theta)=O\left(J(\theta)-\min\limits_{\theta\in\C}J(\theta)+\frac{\ltwo{\C}^4\log(1/\gamma)}{\Delta n}\right).$$
Here $\Delta=\min\limits_{j\in[p]}{\E\limits_x\left[x(j)^2\right]}$.
\label{thm:fastStrongObj}
\end{thm}
From \eqref{eq:ambc1321} and Theorem \ref{thm:fastStrongObj}, we obtain the required bound.
\end{proof}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout"
%%% End:


==> tex/dropoutStabBackup.tex <==
\section{Stability and privacy of dropout for convex learning problems}\label{sec:stabDropout}

In the previous section we saw how dropout ensures that the local minima encountered during the gradient descent are non-robust, and with constant probability gradient descent comes out of it. In this section we demonstrate a dichotomy. We show that for a class of convex learning problems (more precisely, generalized linear models (GLMs)), dropout ensures that the model that globally optimizes the learning objective is robust (stable). In the following we define precisely, what we mean by stability.

Stability is a fundamental property of learning algorithms. Recent works \cite{SSSS,shalev2010learnability,PogVoiRos11,BousquetElisseeff-2002,BST} have shown that stability is both \emph{necessary} and \emph{sufficient} for any learning algorithm. We study two variants of stability: \emph{model stability} and \emph{measure stability}. The former ensures that the model does not change too much (under some distance metric) due addition or deletion of a few training samples, while the latter enforces a stronger property that the induced probability measure on the space of models by any (randomized) algorithm does not change too much. Both model stability and measure stability for an algorithm along with low training error, ensures low generalization error \cite{SSSS,BST}. Furthermore,  measure stability in particular has a direct implication towards differential privacy. At an intuitive level, stability provably ensures that a learning algorithm does not over-fit to ``noise'' in the training data.  In this section we study the stability properties of the dropout heuristic, and in Section \ref{sec:convDiffPrivate} we relate them to differential privacy. In the following, we define the two measures of stability that we study for the dropout method:

\begin{defn}[$\epsilon$-model stability]
	For a given data set $D\in\D^n$ and for any data set $D'\in\D^n$ differing in exactly one entry from $D$, algorithm $\A$ is $\epsilon$-model stable at $D$ if
	$$\E[\ltwo{\A(D)-\A(D')}]\leq \epsilon,$$
	where $\A(D)$ is the output  of $\A$  applied to $D$ and the expectation is over the randomness of $\A$.
	\label{def:modelStab}
\end{defn}

\begin{defn}[$(\epsilon,\delta)$-measure stability]
	For a given data set $D\in\D^n$ and for any neighboring data set $D'\in\D^n$ differing in exactly one entry from $D$, a randomized algorithm $\A$ is $(\epsilon,\delta)$-measure stable at $D$ if for any model parameter $\theta$ drawn from either $\A(D)$ or $\A(D')$, the following holds (with probability  $\geq 1-\delta$):
	$$e^{-\epsilon}\mu_{\A(D')}(\theta)\leq\mu_{\A(D)}(\theta)\leq e^\epsilon\mu_{\A(D')}(\theta).$$
	$\mu_X(\cdot)$ refers to the measure induced by the random variable $X$.
	\label{def:measureStab}
\end{defn}
Throughout the paper we assume that the failure probability $\delta$ is be $1/{\sf poly}(n)$, where ${\sf poly}(n)$ is a polynomial in $n$ of degree at least two. Definition \ref{def:measureStab} implies that for any measurable set $S$ and for any $D'\in\D^n$ that differs from $D$ in exactly one entry, the following holds:
\begin{equation}
e^{-\epsilon}\Pr[\A(D')\in S]-\delta\leq\Pr[\A(D)\in S]\leq e^\epsilon\Pr[\A(D')\in S]+\delta.
\label{eq:meas12}
\end{equation}
\eqref{eq:meas12} is  similar to the notion of $(\epsilon,\delta)$-differential privacy (see Definition \ref{def:diffPrivacy} and
%also implies $(2\epsilon,\frac{\delta}{\epsilon e^\epsilon})$-measure stability (see
\cite[Lemma 3]{DBLP:journals/corr/abs-0803-3946}).

\subsection{Interlude: Dropout stability for linear losses over the simplex}\label{sec:linLoss}
To begin with in this section, we analyze a \emph{stylized} example:  Linear loss functions over the simplex. We show that dropout in this setting actually exhibits measure stability, which is the stronger variant.

Let the data domain $\mathcal{X}$ be $\{0,1\}^p$ and let $X = \{x_1 \dots, x_n\}$ be i.i.d.~samples from a distribution $\tau(\mathcal{X})$ over $\mathcal{X}$. Let the loss function $\ell$ be $\ell(\ip{\theta}{x})=\ip{\theta}{x}$ and let the constraint set $\C$ be the $p$-dimensional simplex. Let $b_1,\cdots,b_n$ be i.i.d. uniform samples from $\{0,1\}^p$. The dropout optimization problem for the linear case can be defined as
\begin{equation}\label{eq:dropLin}
	\nptheta=\arg\min\limits_{\theta\in\C}\sum\limits_{i=1}^n\ip{x_i*b_i}{\theta}
\end{equation}

At a high level Theorem \ref{thm:dropoutStab} states that changing any one data entry in the training data set $D$, changes the induced probability measure on the set of possible outputs by a factor of $\epsilon$, and with a additive slack that is exponentially small in the number of data samples ($n$). See Appendix \ref{app:lindropoutStab} for a proof.

\begin{thm}[Measure stability, linear loss over simplex]
	Let $c(j)=\min\limits_{k\in[n]}\frac{1}{n}\sum\limits_{i=1, i\neq k}^n x_i(j)$ and $\Lambda=\min\limits_{j\in[p]} c(j)$. For the given data set $X$ if $\Lambda>1/(n\epsilon)$ and $\epsilon<1$, then the solution $\nptheta$ of dropout ERM \eqref{eq:dropLin}) is $(\epsilon,\delta)$-measure stable at $X$, where $\delta=p\exp\left(-\Omega(\epsilon^2\Lambda n)\right)$.
	\label{thm:dropoutStab}
\end{thm}


\subsection{Dropout stability for GLM regression}\label{sec:dropoutQuadratic}
To generalize our stability result for linear losses to the generic GLM regression setting we first provide a model stability result for the dropout-based SGD. (For the stability bound of dropout-based ERM, see Section \ref{app:stabERM}.) At a high-level Theorem \ref{thm:modelSGD} ensures that if the dropout SGD (from Section \ref{sec:SGDDrop}) is executed for $T=n^2$ iterations, then by changing any one data entry in the training data set only changes the model by at most $1/n$ (in the $L_2$-norm).
\begin{thm}[Model stability of SGD]
	Let $\C\subseteq\re^p$ be a fixed convex set and let the data domain $\D$ and loss $\ell$ satisfy Assumption \ref{assump:normDat} with parameters $G$, $B$. Let $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ be $n$ samples from $\D$, and let $\Lambda=\frac{1}{n}\min\limits_{k\in[n]}\min\limits_{j\in[p]}\sum\limits_{i=1,i\neq k}^n x_i(j)^2$ and learning rate $\eta_t=\frac{1}{\Delta_1 t}$. Let $T$ be the number of time steps for which SGD (in Section \ref{sec:SGDDrop}) is executed. Then SGD with dropout is $\epsilon_{mod}$-model stable, where $\epsilon_{mod}=O\left(\frac{GB}{\Lambda}\left(\sqrt{\frac{\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{T}}+\frac{1}{n}\right)\right)$. %Here $G$ and $B$ are parameters from Assumption \ref{assump:normDat}.
	\label{thm:modelSGD}
\end{thm}
Here we want to highlight two interesting properties of this theorem: i) stability guarantee holds even if all the data points ($x_i$'s) are aligned in the same direction, i.e., when the Hessian is rank deficient, and ii) the rate of stability is similar to the one that can be obtained by adding an $L_2$-regularizer \cite{CMS11,KST12}.
 
%{\bf  From Model Stability to Measure Stability}:
Unlike in Section \ref{sec:linLoss}, we are only able to show model stability for GLMs. One can see that measure stability cannot be achieved in general for this setting because the support of the distribution over the output model can be different for neighboring data sets and the randomness is multiplicative. However, by modifying the gradient descent algorithm in Section \ref{sec:SGDDrop} to add random perturbation one can achieve measure stability. Specifically we use the Gaussian mechanism from the differential privacy literature (\cite[Lemma 4]{nikolov2013geometry} and Appendix \ref{app:background}). But in order to add the Gaussian perturbation, we need Theorem \ref{thm:modelSGD} to hold w.h.p. We use boosting scheme to achieve this.

\mypar{Boosting of stability} Let $\theta_T^{(1)},\cdots,\theta_T^{(k)}$ be the models from $k$ independent runs of the dropout SGD algorithm (see Section~\ref{sec:SGDDrop}). Let $j^*=\arg\min\limits_{j\in[k]}J(\theta_T^{(j)};D)$, where $J(\theta;D)=\frac{1}{n}\sum\limits_{i=1}^n\E\limits_{b\sim\{0,1\}^p}\left[\ell(2\ip{x_i*b}{\theta};y_i)\right]$. If $k=\log(1/\delta)$, then w.p. $\geq 1-\delta$, we have: $\ltwo{\theta^{(j^*)}_T(D)-\theta^{(j^*)}_T(D')}\leq \epsilon_{mod}\sqrt{\log(1/\delta)}$, where $\epsilon_{mod}$ is defined in Theorem \ref{thm:modelSGD} (see Appendix \ref{app:highProbModStab} for more details).

Now, using standard results from differential privacy literature \cite{nikolov2013geometry}, we can show that $\hat\theta_T=\theta_T^{(j^*)}+\mathcal{N}(0,\I_p\frac{\epsilon_{mod}^2\cdot \log(1/\delta)}{\epsilon})$ is $(\epsilon,\delta)$-{\em measure stable} at the data set $D$. Furthermore, using the fact that $\rL(\theta)$ is $O(GB)$ Lipschitz and the results of \cite[Theorem 1]{jain2014near} and \cite[Theorem 3]{CMS11}, we have:
 %, using the properties of Gaussian random variables and the fact that we are in the GLM setting, the following two guarantees are true in expectation (over the randomness of the Gaussian noise distribution). These bounds follow from
%the results of \cite[Theorem 1]{jain2014near} and \cite[Theorem 3]{CMS11} respectively.
%Let $\sigma=O\left(\frac{GB\log(1/\delta)}{\epsilon\Lambda}\left(\sqrt{\frac{\log T\max\{\Delta_1/\Lambda,\Lambda/\Delta_1\}}{T}}+\frac{1}{n}\right)\right)$. Now using the result from Gaussian mechanism \cite{nikolov2013geometry} one can show that  $\hat\theta_T=\theta_T^{(j^*)}+\mathcal{N}(0,\I_p\sigma^2)$ is $(\epsilon,\delta)$-measure stable at the data set $D$. (See Appendix \ref{app:background} for more details on Gaussian mechanism.) If there is strict requirement of outputting a vector in $\C$ (i.e., in a \emph{proper learning} setting), then one can project $\hat\theta_T$ to $\C$ while preserving the same measure stability guarantee. Using the definition of $\rL(\theta)$ from \eqref{eq:risk12}, we have the following.
%Since $\rL(\theta)$ is $O(GB)$ Lipschitz, using the properties of Gaussian random variables and the fact that we are in the GLM setting, the following two guarantees are true in expectation (over the randomness of the Gaussian noise distribution). These bounds follow from the results of \cite[Theorem 1]{jain2014near} and \cite[Theorem 3]{CMS11} respectively.
\begin{enumerate}\itemsep -3pt
    \item \textbf{Improper learning bound:} $\E[|\rL(\hat\theta_T^{(j^*)})-\rL(\theta_T^{(j^*)})|]=G\sigma$.
    \item \textbf{Proper learning bound:} $\E[|\rL(\proj_\C(\hat\theta_T^{(j^*)}))-\rL(\theta_T^{(j^*)})|]=GB\sqrt{p}\sigma $.
\end{enumerate}

Notice that the improper learning bound is independent of any \emph{explicit} dependence on $p$. Also if $T=n^2$ and if we consider $\Lambda$ and all parameters except $n$ to be constants, then the above bounds indicate that the excess error due to the Gaussian noise addition is $O\left(1/n\right)$, which is similar to the excess risk bound of the standard dropout algorithm (Theorem \ref{thm:dropoutGen}). Using arguments similar to \cite{BST} one can show that this bound is tight.

\mypar{Optimality of error} Regularized private risk minimization is a well-studied area \cite{CM08,DL09,CMS11,JKT12,KST12,DuchiJW13,song2013stochastic,jain2014near,BST}. Here we provide yet another algorithm for private risk minimization. While the previous algorithms primarily used variants of $L_2$ regularization, we use the dropout regularization for the privacy guarantee. Conditioned on the PTR test passing, the utility of this algorithm follows from the learning bounds obtained for the measure stable version of dropout which depends on the noise level $\sigma$. While the bounds are tight in general \cite{BST} and there exists other algorithms achieving the same bounds \cite{BST,jain2014near}, since dropout has been often shown to outperform vanilla regularization schemes, it might be advantageous to use dropout learning even in the context of differential privacy. (See Section \ref{sec:experiments} for more discussions.)  


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout_nips"
%%% End:


==> tex/genPerfStab.tex <==
\section{Applications of measure stability results}
We now discuss two important applications of our measure stability results, that further establish dropout algorithm's usefulness in practice. 

\input{tex/convDropDiff}

\subsection{Implications of stability on generalization performance}
\label{Sec:stabGenPerf}

Both model stability and measure stability have direct implications on generalization error. $\epsilon$-model stability implies that changing $m$ entries in the data set adversarially, only changes the excess risk by $O(m\epsilon)$. $(\epsilon,\delta)$-measure stability implies even a stronger property: For any data set $D'$ differing in at most $m$ entries from $D$, the following is true.
$$\E\limits_{\A}\left[{\sf Risk}(\A(D'))\right]\leq e^{m\epsilon}\E\limits_{\A}\left[{\sf Risk}(\A(D))\right]+mB\delta.$$
Here $B$ is an upper bound on the $L_2$-norm of the feature vectors. Since, $\delta$ is $1/{\sf poly}(n)$, this gives a multiplicative closeness on the excess risk. For a more formal treatment, see Appendix \ref{app:stabGenPerf}.

Note that for $L_2$-regularized ERM, the corresponding excess risk bound under adversarial corruption is: ${\sf Risk}(\A(D'))\leq {\sf Risk}(\A(D))+m/(n\lambda),$ where $\lambda$ is the regularization parameter. Now, if the risk of $\A(D)$ is small (say for separable dataset), then our risk bound for dropout is as small as $1/poly(n)$, while $L_2$ regularized ERM still has excess risk at rate $1/n$. However, for ${\sf Risk}\A(D)$, dropout bound can be significantly worse than that of $L_2$-regularized ERM. 

%Next, we show that measure-stability of our dropout based approach provides small excess risk bounds even when a small number of points are corrupted adverserially. The key idea behind our approach is that due to multiplicative closeness in distribution of $\nptheta(D)$ and $\nptheta(D')$ ($D, D'$ differ in only one entry), $f(\nptheta(D))$ and $f(\nptheta(D'))$ are both close (assuming $f$ is Lipschitz). Formally, we have;
%In this section we focus on the following question: \emph{What implication does stability have on the generalization performance?} There is a large body of literature answering this question under different measures of stability. (See \cite{shalev2010learnability} for a survey.) For a large class of problem settings, the notions of stability we consider in this paper are stronger than almost all the other measures stated in the literature. Instead of a comparison between various measures of stability, we show the following connection to generalization error and risk.
%For a given data set $D$ and an algorithm $\A$, let \emph{distance to $(\epsilon,\delta)$-measure instability} be the minimum number of entries in $D$ that needs to be changed to form a data set $D'$ such that $\A$ is not $(\epsilon,\delta)$-measure stable at $D'$. Analogously define the distance to \emph{$\epsilon$-model instability} at data set $D$. We show that for any function $f:\C\to\re$ executed on $\A(D)$ and $\A(D')$ such that $D'$ is within the distance to instability, $f(\A(D))$ and $f(\A(D'))$ are ``close''. For precise measures of closeness see Theorems \ref{thm:modelStab12} and Theorem \ref{thm:measureStab12} respectively.
%Notice that since $\delta$ is typically very small (around $1/{\sf poly}(n)$, Theorem \ref{thm:measureStab12} provides ``nearly'' multiplicative closeness. Also notice that we have very little assumption on the function $f$. In particular, $f$ can be any reasonable measure of risk (or generalization error) (e.g., ${\sf Risk}$ or ${\sf ExcessRisk}$ in Section \ref{sec:probDef}).
%\begin{thm}
%Let $f:\C\to\re$ be a $L$-Lipschitz continuous function. For a given data set $D\in\D^n$, if an algorithm $\A$ (with the range space of $\A$ in $\C$) has $\Gamma$ distance to $\epsilon$-model instability, then for any data set $D'$ differing in at most $m<\Gamma$, the following holds:
%\begin{equation}
%$\E\limits_{\A}\left[\left|f(\A(D))-f(\A(D'))\right|\right]\leq Lm\epsilon.$
%\label{eq:modelStabaswee}
%\end{equation}
%\label{thm:modelStab12}
%\end{thm}
%The proof Theorem \ref{thm:modelStab12} above follows immediately by triangle inequality.

%\begin{thm}
%Let $f:\C\to\re$ be a bounded function with $\max\limits_{x\in\C} |f(x)|\leq B$. For a given data set $D\in\D^n$, if an algorithm $\A$ (with the range space of $\A$ in $\C$) has $\Gamma$ distance to $(\epsilon,\delta)$-measure instability, then for any data set $D'$ differing in at most $m<\Gamma$, the following holds.
%\begin{equation}
%\E\limits_{\A}\left[f(\A(D))\right]\leq e^{m\epsilon}\E\limits_{\A}\left[f(\A(D'))\right]+mB\delta.
%\label{eq:kjh1234}
%\end{equation}
%\label{thm:measureStab12}
%\end{thm}
%{\bf Importance of the result}:???

%The proof of Theorem \ref{thm:measureStab12} follows immediately by union bound and multiplicative closeness of measures. To get more insight into the distance to instability, we consider the following setting. For the ease of exposition, we assume the number of dimensions $p$ to be a constant and ignore ${\sf poly} \log$ terms in $n$, and hide them in the $\tilde O(\cdot)$ notation.

%\mypar{Example} Consider a model vector $\theta^*\in\C$ and a distribution $\mathcal{N}(0,\Sigma^{-1})$, where $\Sigma$ is a diagonal covariance matrix with the diagonal being $\langle\lambda_1^2,\cdots,\lambda_p^2\rangle$. And let $D=\{(x_1,y_1),\cdots,(x_n,y_n)\}$ be a data set of $n$ entries, where each $x_i\sim \mathcal{N}(0,\Sigma^{-1})$ and $y_i=\ip{x_i}{\theta^*}$. For dropout regularization, the corresponding optimization problem is given in \eqref{eq:dropout}.

%Let $\Lambda_\Gamma=\frac{1}{n}\left[\min\limits_{S\subseteq[n],|S|=\Gamma}\min\limits_{j\in[p]}\sum\limits_{i=1,i\not\in S}^n x_i(j)^2\right]$. Intuitively, $\Lambda_\Gamma$ refers to the strong convexity of the expected objective function in \eqref{eq:dropout}, when at most $\Gamma$ entries are adversarially modified in the data set $D$. By the tail bound for Chi-squared distribution, one can show that $\Lambda_\Gamma=\Omega(1)$ with probability at least $1-1/{\sf poly}(n)$ as long as $\lambda_1,\cdots,\lambda_p$ are $\Omega(1)$ and $\Gamma=\tilde o(n)$. Therefore, for a given value of $\epsilon$ and $\delta$ and any data set $D'$ such that $|D\Delta D'|\leq 2\Gamma$, the standard deviation $\sigma$ of the noise needed to obtain $(\epsilon,\delta)$-measure stability in Section \ref{sec:modelToMeasure} is $ \widetilde O\left(\frac{\log(1/\delta)}{\epsilon n}\right)$. This implies that for the above value of $\sigma$, \eqref{eq:kjh1234} in Theorem \ref{thm:measureStab12} is true for all $m=\tilde o(n)$.

%Similarly for model stability, one can show for $m=\tilde o(n)$ in the above example, \eqref{eq:modelStabaswee} in Theorem \ref{thm:modelStab12} is true with $\epsilon=\tilde O(1/n)$.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../StableDropout_nips"
%%% End:


==> tex/outline.tex <==
\section{Outline}
Abstract and intro: 
\begin{itemize}
\item We study dropout for the convex ERM
\item We show that dropout in fact optimizes a regularized strongly convex loss function
\item We provide generalization error bounds for it
\item More interestingly, we show that dropout with a small Gaussian noise satisfies a very strong notion of stability called measure stability
\item We show that measure stability is important because it ensures robustness to even adverserial noise
\item Using this connection, we provide exact noise robustness for dropbout+gaussian noise based algorithm
\item We show empirically that dropout indeed performs better than simple gardient descent even for convex loss functions
\end{itemize}

Related works: 
\begin{itemize}
\item percy liang, and one other
\item dropout is very popular in DNN
\item stability is important by niyogi
\item differential privacy connections (smith and thakurta, online diff privacy)
\end{itemize}

problem setup and notations: 
GLM model, iid data, lipschitz functions 

Dropout generalization error analysis: 
we study this type of dropout algorithm, show generalization error wrt a ``expecc`ted loss function''. Then for least squares, we show it is optimizing a L2 regualrized loss function

Stability of Dropout: 
Notions of stability and their connections to Niyogi's notions
Stability of dropout
robustness to adverserial noise by dropout: first we general result that if an algroithm is measure stable, then it is stable to adverserial noise and then show that dropout indeed is robust

Experiments: 
simplest experiment: least squares on 2-3 benchmark datasets (kdd cup, URL dataset). Show that dropout is better than simple gradient descent and similar to L2 regularized gradient descent. 

neural network experiment: dropout is better than L2 regularized gradient descent and L2 reg. noisy gradient descent as well (MNIST dataset)

robustness experiment: change yi to T-yi (T is the max value of target variables yi's) or change it to another random yi.  (MNIST, KDD cup, URL dataset)

Non-convex experiment: neural network, add 10 points at each stage and see generalization error on a fixed validation set for droput as well as L2 reg. gradient descent (MNIST, KDD cup, URL dataset). 




%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "../StableDropout"
%%% End: 


==> tex/related.tex <==
\section{Survey of Related Works}
\label{sec:relatedWork}
